TabFlex: Scaling Tabular Learning to Millions with Linear Attention

Leveraging the in-context learning (ICL) capability of Large Language Models (LLMs) for tabular classification has gained significant attention for its training-free adaptability across diverse datasets. Recent advancements, like TabPFN, excel in small-scale tabular datasets but struggle to scale for large and complex datasets. Our work enhances the efficiency and scalability of TabPFN for larger datasets by incorporating linear attention mechanisms as a scalable alternative to complexity-quadratic self-attention. Our model, TabFlex, efficiently handles tabular datasets with thousands of features and hundreds of classes, scaling seamlessly to millions of samples. For instance, TabFlex processes the poker-hand dataset with over a million samples in just 5 seconds. Our extensive evaluations demonstrate that TabFlex can achieve over a 2x speedup compared to TabPFN and a 1.5x speedup over XGBoost, outperforming 25 tested baselines in terms of efficiency across a diverse range of datasets. Furthermore, TabFlex remains highly effective on large-scale datasets, delivering strong performance with significantly reduced computational costs, especially when combined with data-efficient techniques such as dimensionality reduction and data sampling.

==> archive.tex <==
\section{Unused Tables}
\begin{table}[]
\centering
 \resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|cccccc|cccccc}
\toprule
 \multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\textbf{\#Classes}} & \multirow{2}{*}{\textbf{\#Features}} & \multirow{2}{*}{\textbf{\#Instances}} & \multicolumn{6}{c|}{\textbf{Mean ROC AUC}} & \multicolumn{6}{c}{\textbf{Mean Time (s)}} \\ 

 & & & & CatBoost & MLP & TabNet & ResNet & \tabpfn{} & \ours{} & CatBoost & MLP & TabNet & ResNet & \tabpfn{} & \ours{} \\
\midrule
SpeedDating & 1 & 120 & 8378 & 0.864 & 0.846 & 0.829 & 0.863 & 0.547 & 0.848 & 12.040 & 13.057 & 150.625 & 11.007 & 1.585 & 1.526 \\
audiology & 24 & 69 & 226 & 0.875 & 0.650 & 0.616 & 0.923 & 0.818 & 0.845 & 54.556 & 5.122 & 7.441 & 4.921 & 0.233 & 0.218 \\
cnae-9 & 9 & 856 & 1080 & 0.990 & 0.996 & 0.984 & 0.994 & 0.479 & 0.914 & 1.767 & 10.502 & 26.578 & 5.593 & 0.507 & 3.099 \\
jasmine & 1 & 144 & 2984 & 0.871 & 0.852 & 0.823 & 0.854 & 0.704 & 0.851 & 1.678 & 6.058 & 61.822 & 4.405 & 1.273 & 0.767 \\
nomao & 1 & 118 & 34465 & 0.992 & 0.991 & 0.992 & 0.993 & 0.762 & 0.986 & 4.211 & 86.451 & 517.712 & 70.047 & 1.818 & 4.167 \\
\bottomrule
\end{tabular}
}
\caption{Caption}
\label{tab:my_label}
\end{table}

\begin{table}[]
\centering
 \resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|cccccc|cccccc}
\toprule
 \multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\#Classes} & \multirow{2}{*}{\textbf{\#Features}} & \multirow{2}{*}{\textbf{\#Instances}} & \multicolumn{6}{c|}{\textbf{Mean ROC AUC}} & \multicolumn{6}{c}{\textbf{Mean Time (s)}} \\ 

 & & & & CatBoost & MLP & TabNet & ResNet & \tabpfn{} & \ours{} & CatBoost & MLP & TabNet & ResNet & \tabpfn{} & \ours{} \\
\midrule
MiniBooNE & 2 & 50 & 130064 & 0.978 & 0.978 & 0.927 & 0.969 & 0.977 & 0.974 & 2.605 & 265.559 & 699.083 & 447.403 & 3.194 & 7.222 \\
airlines & 2 & 7 & 539383 & 0.698 & 0.651 & - & 0.705 & 0.628 & 0.639 & 4.510 & 511.987 & - & 571.425 & 9.728 & 4.195 \\
albert & 2 & 78 & 425240 & 0.768 & 0.654 & - & 0.756 & 0.686 & 0.701 & 33.980 & 405.528 & - & 490.106 & 9.390 & 13.461 \\
higgs & 2 & 28 & 98050 & 0.787 & 0.793 & - & 0.812 & 0.724 & 0.756 & 1.999 & 222.441 & - & 199.242 & 2.818 & 4.920 \\
poker-hand & 10 & 10 & 1025009 & 0.839 & 0.539 & - & - & 0.718 & 0.837 & 355.365 & 504.520 & - & - & 15.364 & 4.879 \\
\bottomrule
\end{tabular}
}
\caption{Caption}
\label{tab:my_label}
\end{table}

\begin{table}[htbp]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{l|rrr|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\#Features}} & \multirow{2}{*}{\textbf{\#Instances}} & \multirow{2}{*}{\textbf{\#Classes}}  & \multicolumn{2}{c|}{\textbf{Mean AUC}} & \multicolumn{2}{c}{\textbf{Mean Time (seconds)}} \\ \cmidrule{5-8}
& & & & \tabpfn{} & \ours{} & \tabpfn{} & \ours{} \\
\midrule
fri\_c2\_500\_50 & 51 & 500 & 2 & 0.763 & \textbf{0.926} & \textbf{0.224} & 0.436 \\
micro-mass & 1301 & 571 & 20 & 0.712 & \textbf{0.820} & \textbf{0.575} & 4.796 \\
xd6 & 10 & 973 & 2 & \textbf{1.000} & \textbf{1.000} & \textbf{0.091} & 0.121 \\
kdd\_internet\_usage & 69 & 10108 & 2 & \textbf{0.932} & \textbf{0.932} & 2.013 & \textbf{0.778} \\
stock & 10 & 950 & 2 & \textbf{0.993} & \textbf{0.993} & \textbf{0.119} & 0.142 \\
GTSRB-HOG02 & 1569 & 51839 & 43 & 0.596 & \textbf{0.668} & \textbf{9.092} & 40.142 \\
Kuzushiji-49 & 785 & 270912 & 49 & 0.582 & \textbf{0.631} & 152.276 & \textbf{114.655} \\
Run\_or\_walk\_information & 7 & 88588 & 2 & \textbf{0.998} & 0.996 & 15.100 & \textbf{1.535} \\
one-hundred-plants-margin & 65 & 1600 & 100 & 0.546 & \textbf{0.584} & 1.218 & \textbf{0.543} \\
KDD98 & 478 & 82318 & 2 & 0.574 & \textbf{0.609} & \textbf{18.375} & 24.091 \\
fars & 30 & 100968 & 8 & \textbf{0.872} & \textbf{0.872} & 20.474 & \textbf{2.816} \\
GTSRB-HOG01 & 1569 & 51839 & 43 & 0.596 & \textbf{0.632} & \textbf{9.112} & 41.216 \\
one-hundred-plants-shape & 65 & 1600 & 100 & 0.544 & \textbf{0.567} & 0.990 & \textbf{0.614} \\
porto-seguro & 38 & 595212 & 2 & 0.599 & \textbf{0.619} & 687.326 & \textbf{19.889} \\
hiva\_agnostic & 1618 & 4229 & 2 & 0.762 & \textbf{0.780} & \textbf{1.589} & 7.033 \\
water-treatment & 37 & 527 & 2 & 0.967 & \textbf{0.984} & \textbf{0.223} & 0.321 \\
spoken-arabic-digit & 15 & 263256 & 10 & 0.497 & \textbf{0.507} & 133.021 & \textbf{6.237} \\
compas-two-years & 14 & 5278 & 2 & \textbf{0.734} & 0.730 & 0.245 & \textbf{0.213} \\
autoUniv-au6-750 & 41 & 750 & 8 & 0.501 & \textbf{0.509} & \textbf{0.200} & 0.270 \\
volcanoes-b6 & 4 & 10130 & 5 & 0.654 & \textbf{0.660} & 0.338 & \textbf{0.192} \\
madeline & 260 & 3140 & 2 & \textbf{0.652} & 0.634 & \textbf{1.147} & 1.776 \\
GAMETES\_Epistasis\_2-Way\_1000atts\_0.4H\_EDM-1\_EDM-1\_1 & 1001 & 1600 & 2 & \textbf{0.496} & 0.487 & \textbf{1.012} & 5.324 \\
GTSRB-HueHist & 257 & 51839 & 43 & \textbf{0.571} & 0.551 & \textbf{8.660} & 9.732 \\
bank32nh & 33 & 8192 & 2 & 0.889 & \textbf{0.893} & 1.292 & \textbf{0.480} \\
oil\_spill & 50 & 937 & 2 & 0.942 & \textbf{0.945} & 0.462 & \textbf{0.368} \\
volcanoes-d4 & 4 & 8654 & 5 & 0.628 & \textbf{0.630} & 0.284 & \textbf{0.194} \\
USPS & 257 & 9298 & 10 & \textbf{0.998} & 0.992 & \textbf{2.180} & 2.792 \\
boston\_corrected & 21 & 506 & 2 & 0.943 & \textbf{0.944} & \textbf{0.156} & 0.261 \\
tokyo1 & 45 & 959 & 2 & 0.979 & \textbf{0.979} & 0.311 & \textbf{0.296} \\
fri\_c4\_500\_100 & 101 & 500 & 2 & \textbf{0.684} & 0.676 & 0.530 & \textbf{0.523} \\
tamilnadu-electricity & 4 & 45781 & 20 & \textbf{0.500} & 0.499 & 4.454 & \textbf{1.019} \\
meta\_stream\_intervals.arff & 75 & 45164 & 11 & 0.933 & \textbf{0.983} & 8.539 & \textbf{3.895} \\
GTSRB-HOG03 & 2917 & 51839 & 43 & 0.594 & \textbf{0.638} & \textbf{9.159} & 40.205 \\
led24 & 25 & 3200 & 10 & \textbf{0.946} & 0.944 & 0.776 & \textbf{0.249} \\
\bottomrule
\end{tabular}}
    \caption{Validation set}
    \label{tab:val}
\end{table}

==> etc.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

